Parallel Dynamic Spatial Indexes

Maintaining spatial data (points in two or three dimensions) is crucial and has a wide range of applications, such as graphics, GIS, and robotics. To handle spatial data, many data structures, called spatial indexes, have been proposed, e.g. kd-trees, oct/quadtrees (also called Orth-trees), R-trees, and bounding volume hierarchies (BVHs). In real-world applications, spatial datasets tend to be highly dynamic, requiring batch updates of points with low latency. This calls for efficient parallel batch updates on spatial indexes. Unfortunately, there is very little work that achieves this. In this paper, we systematically study parallel spatial indexes, with a special focus on achieving high-performance update performance for highly dynamic workloads. We select two types of spatial indexes that are considered optimized for low-latency updates: Orth-tree and R-tree/BVH. We propose two data structures: the P-Orth tree, a parallel Orth-tree, and the SPaC-tree family, a parallel R-tree/BVH. Both the P-Orth tree and the SPaC-tree deliver superior performance in batch updates compared to existing parallel kd-trees and Orth-trees, while preserving better or competitive query performance relative to their corresponding Orth-tree and R-tree counterparts. We also present comprehensive experiments comparing the performance of various parallel spatial indexes and share our findings at the end of the paper.

==> Implementation.tex <==
\section{Implementation Details}
\label{sec:impl}
\myparagraph{\ourorth{}.}
We implement the \ourorth{} based on the \pkd{}~\cite{xxx}.


==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> batch_delete_algorithm.tex <==
\setlength{\algomargin}{0em}
\begin{algorithm}[t]
	\fontsize{8pt}{8.5pt}\selectfont
	\caption{Batch deletion\label{batchdelete}}
	\SetKwFor{parForEach}{parallel-foreach}{do}{endfor}
	\KwIn{Points $P$ with dimension $k$, a $k$d-tree $T$.}
	\KwOut{A $k$d-tree with $P$ deleted.}
	\SetKw{MIN}{min}
	\SetKw{MAX}{max}
	\SetKwProg{MyFunc}{Function}{}{end}
	\SetKwInOut{Note}{Note}
	\SetKwFor{inParallel}{in parallel:}{}{}
	\SetKwInOut{Parameter}{Parameter}
	\Parameter{$\skheight$: the maximum height of a fetched tree skeleton.\\
		$\leafwrap$: the leave wrap of $T$.
	}
	%	 \vspace{0.5em}
	\DontPrintSemicolon
	\vspace{.5em}
	\tcp{Delete points $P$ from a $k$d-tree $T$. Boolean flag $t$ takes value $1$ if none of $T$'s ancestor needs rebuild after deletion and 0 otherwise. }
	\MyFunc{\upshape{\batchdelete$(P,T,t)$}}{
		$n\gets |P|$\tcp*[f]{Size of the input batch}\\
		\If{$n=0$}{\Return $T$}
		\If{$T$ is leaf}{
			$T.p\gets T.p\setminus P$\tcp*[f]{Remove the points from the leaf}\label{removeFromLeave}\\
			\Return $T$	
		}
		$\matht \gets \fetchTreeSkeleton(T,0)$\label{fetchTreeSkeleton}\\
		Sieve points to the corresponding bucket node in $\matht$, array slice $B[i]$ holds all points sieved to bucket node $i$.\label{sieveDelete}\\
		Put a tomb to the (sub)tree in $\matht$ if it becomes imbalance after deletion. If both a node and its ancestor are imbalance, put the tomb to its ancestor only\label{puttomb}\\
		\tcp{Delete the points from subtrees of $T$ first}
		\parForEach{bucket id $i$}{
			$\matht_i\gets$ bucket node with identifier $i$\\
			\eIf(\tcp*[f]{Any subtree containg $\matht_i$ is balance})
			{$\matht_i$ has tomb}
			{$T_i=\batchdelete(B[i],\matht_i,1)$\label{withTomb}}
			(\tcp*[f]{Some subtrees containg $\matht_i$ will be rebuilt})
			{$T_i=\batchdelete(B[i],\matht_i,0)$\label{noTomb}}
			Replace the node $\matht_i$ in $\matht$ with $T_i$ and redirect its parent's pointer to $T_i$ 
		}
		\tcp{Rebuild imbalance nodes then}
		$U\gets$ Set of nodes in $\matht$ that hold a tomb\\
		\parForEach{$\varmatht\in U$\label{beginRebuildDelete}}{
			 $\varmatht'\gets\build(\{q\})$\label{rebuildINDelete}\\
			 Replace node $\varmatht$ in $\matht$ with $\varmatht'$\\
			$\deleteTree(\varmatht)$\label{endRebuildDelete}
		}
		\Return The root of $\matht$ $\label{returnSkDeletion}$
	}
	\end{algorithm}


==> batch_dynamic.tex <==
\section{Parallel Algorithms for Batch Updates \label{sec:update}}


==> construct-analysis.tex <==
\subsection{Theoretical Analysis}\label{sec:constr-analysis}

We now formally analyze our construction algorithm and show its theoretical efficiency.
%We start with some useful lemmas. We first show a conclusion
We start with a useful lemma about sampling.
Similar results about sampling have also been shown previously \cite{RR89,agarwal2016parallel,blelloch2018geometry}.
We put it here for completeness.

\begin{lemma}\label{lem:sampling}%[Sampling]
  For a \ourkdtree $T$ with size $n'$,
  for any $\epsilon<1$,
  setting $\os=(6c\log n)/\epsilon^2$ guarantees that the size of a child subtree is within the range of $(1/2\pm \epsilon/4)\cdot n'$ with probability at least $1-2/n^c$.
\end{lemma}
Here we need to distinguish a subtree size $n'$ and the overall tree size $n$ for a stronger high probability guarantee, so we can apply union bounds in the later analysis.
\medskip
\begin{proof}
  %We first show that by setting $\os=(12c\log n)/\epsilon^2$, the probability that the child subtree sizes drop below $(1/2 - \epsilon/4)\cdot n'$ is no more than $1/n^c$.
  %We first consider the left subtree $T.lc$, and the other case is symmetric.
  \cref{algo:constr} guarantees that each leaf in a skeleton has at least $\os$ sampled points.
  Therefore, every time we find a splitter,
  it is the median of at least $2\os$ sampled points.
  Let $s$ ($\ge 2\os$) be the number of samples for this \ourkdtree $T$,
  and $\Lambda\subset T$ contains the smallest $(1/2 - \epsilon/4)\cdot n'$ points in the cutting dimension.
  We want to show that the chance we have more than $s/2$ samples in $\Lambda$  (i.e., the left side has fewer than $(1/2 - \epsilon/4)\cdot n'$ points) is small.
  Since all samples are picked randomly, we denote indicator variable $X_i$, where $X_i=1$ if the $i$-th sample is in $\Lambda$ and 0 otherwise.
  Let $X=\sum X_i$ for $i=1..|\Lambda|$, and $\mu = \mathbb E[X] = (1/2-\epsilon/4)s$.
  Let $\delta = \epsilon/(2-\epsilon)$. Then $(1+\delta)\mu=(1+\frac{\epsilon}{2-\epsilon})(\frac{1}{2}-\frac{\epsilon}{4})s=\frac{s}{2}$.
  Using the form of Chernoff Bound $\Pr[X\geq (1+\delta)\mu]\leq \exp(-{\delta^2\mu}/(2+\delta))$,
  we have:
  \begin{align*}
    \Pr\left[X\geq \frac{s}{2}\right] & \leq \exp\left(-\frac{\delta^2\mu}{2+\delta}\right) = \exp\left(-\frac{\epsilon^2 s}{16-4\epsilon}\right)                    & \hfill\!\!\!\!\!\!\!\!\!\!\!(\text{plug in }s\ge 2\os) \\
    & \le\exp\left(-\frac{12c\log n}{16-4\epsilon}\right)=\frac{1}{n^{c\cdot{\frac{12\log_2 e}{16-4\epsilon}}}} \le \frac{1}{n^c}.
  \end{align*}
  The right subtree has the same low probability of being unbalanced, so taking the union bound gives the state bound.
\end{proof}


\hide{
  \begin{lemma}[Sampling]\label{lem:sampling}
    For a \ourkdtree $T$ with size $n'$, setting $\os=\Omega((\log n)/\epsilon^2)$ guarantee a child subtree within $(1/2\pm \epsilon/4)\cdot n'$ nodes for any $\epsilon<1$ \whp{} in $n$.
    %\whp in terms of $n$ for $\os=\Omega(\log n)$ and any $\epsilon =\sqrt{(12c\log n)/\os}<1$.%with probability at least $1-n^{-c}$
  \end{lemma}
  Here we need to distinguish a subtree size $n'$ and the overall tree size $n$ for a stronger high probability guarantee, so we can apply union bounds in the later analysis.
  \medskip
  \begin{proof}
    We show that by setting $\os=(12c\log n)/\epsilon^2$, the probability that the child subtree sizes drop below $(1/2\pm \epsilon/4)\cdot n'$ is no more than $1/n^c$.
    This is equivalent to the statement in the lemma.
    We first consider the left subtree $T.lc$, and the other case is symmetric.

    In \cref{algo:constr}, every time we find the pivot, it is the median of at least $\os$ sampled points.
    Here let $s$ ($\ge \os$) be the sample size of this \ourkdtree (the current subtree), and $S'$ contains the smallest $(1/2\pm \epsilon/4)\cdot n'$ points in the cutting dimension.
    We want to show that the chance we have more than $s/2$ samples in $S'$ is small.
    Since all samples are picked randomly, we denote indicator variable $X_i=1, i\in S'$ if $i$-th sample is in $S'$ and 0 otherwise.
    Let $X=\sum_{i\in S'}X_i$ and $\mu = \mathbb E[X] = (1/2-\epsilon/4)s$.
    Let $\delta = \epsilon/(2-\epsilon)$, and we have $(1+\delta)\mu=(1+\frac{\epsilon}{2-\epsilon})(\frac{1}{2}-\frac{\epsilon}{4})s=\frac{s}{2}$.
    Using the form of Chernoff Bound $P[X\geq (1+\delta)\mu]\leq \exp(-{\delta^2\mu}/(2+\delta))$,
    we have:
    \begin{align*}
      \mathbb P[X\geq \frac{s}{2}] & \leq \exp\left(-\frac{\delta^2\mu}{2+\delta}\right) = \exp\left(-\frac{\epsilon^2 s}{16-4\epsilon}\right)                  \\
      & \le\exp\left(-\frac{12c\log n}{16-4\epsilon}\right)=\frac{1}{n^{c\cdot{\frac{12\log e}{16-4\epsilon}}}} \le \frac{1}{n^c}.
    \end{align*}
    The right subtree has the same low probability to be unbalanced, so taking the union bound gives the stated bound.
    %Similarly, there are less than $s/2$ points from $P_R$ in $S$ \whp. The proof follows by the union bound.
    \hide{
      We can partition the input points $P$ into three groups:
      \begin{itemize}
        \item $P_L = \{x\in P: rank(x)\leq n/2-\epsilon/4\}$
        \item $P_M = \{x\in P: n/2-\epsilon/4 < rank(x) < n/2+\epsilon/4\}$
        \item $P_R = \{x\in P: rank(x)\geq n/2+\epsilon/4\}$
      \end{itemize}
      Let $s=|S|$ the sample size. If fewer than $s/2$ points from both $P_L$ and $P_R$ are presented in $S$, then the median from $S$ is the desired one. Denote indicator variable $X_i=1, i\in S$ if $i$-th sample is in $P_L$ and 0 otherwise. Let $X=\sum_{i\in S}X_i$ and $\mu = \mathbb E[X] = (1/2-\epsilon/4)s$. We have:
      % \begin{align}
      %   \mu = \mathbb E[X] = \sum_{i\in S}\mathbb E[X_i] =\sum_{i\in S}\mathbb P(X_i=1) = s\cdot(1/2-\epsilon/4)
      % \end{align}
      \begin{align}
        \mathbb P[X\geq \frac{s}{2}] & = \mathbb P[X\geq (\frac{1}{2}-\frac{\epsilon}{4})s+\frac{\epsilon}{4}s]           \\
        & =\mathbb P[X\geq (1+\frac{\epsilon}{2-\epsilon})(\frac{1}{2}-\frac{\epsilon}{4})s] \\
        & =\mathbb P[X\geq (1+\delta)\mu]
      \end{align}
      where $\delta = \epsilon/(2-\epsilon)$. Using First Chernoff Bound, we have:
      \begin{align}
        \mathbb P[X\geq \frac{s}{2}] & \leq \exp(-\frac{\delta^2\mu}{2+\delta})        \\
        & = \exp(-\frac{\epsilon^2 s}{16-4\epsilon})      \\
        & =\exp(-\frac{2^\skheight}{16-4\epsilon} \log n) \\
        & = \frac{1}{n^c}
      \end{align}
    where $c=2^\skheight/(\ln2(16-4\epsilon))$. Similarly, there are less than $s/2$ points from $P_R$ in $S$ \whp. The proof follows by the union bound.}
  \end{proof}
}

\begin{lemma}[Tree height]\label{lem:tree-height}
  The total height of a \ourkdtree with size $n$ is $O(\log n)$ for $\os=\Omega(\log n)$, or $\log n+O(1)$ for $\os=\Omega(\log^3 n)$, both \whp.
\end{lemma}
\begin{proof}
  To prove the first part, we will use $\epsilon=1$ in \cref{lem:sampling}.
  In this case, for $\os=6c\log n$, one subtree can have at most 3/4 of the size of the parent with probability $1-1/n^c$, which means that
  the tree size shrinks by a quarter every level. This indicates that the tree heights is $O(\log n)$ \whp for any constant $c>0$.

  We now show the second part of this lemma. For leaf wrap $\leafwrap\ge 4$, the tree has height 1 for $n\leq 4$.
  %By plugging in $\epsilon=O(1)/\log n$, the tree height $h$ can be solved as $\log n+O(1)$.
  We will show that using $\epsilon=4/\log n$  (i.e., $\os=O(\log^3 n)$), the tree height $h$ is $\log n+O(1)$.
  Similar to the above, here in the worst case, for a subtree of size~$n'$, the children's subtree size is at most $(1/2+\epsilon/4)\cdot n'=(1/2+1/\log n)\cdot n'$.
  %For simplicity, we let $\epsilon=4/\log n$ so $1/2+\epsilon/4=1/2+1/\log n$.
  Hence, the tree height satisfies $(1/2+1/\log n)^h=1/n$, so $h={-\log n}/{\log(1/2+1/\log n)}$.
  Here, let $\delta=h-\log n={-\log n}/{\log(1/2+1/\log n)}-\log n$. It solves to $\delta=O(1)$ for $n> 4$.
  Although complicated, the analysis primarily employs some algebraic methods. \ifconference{Due to the space limit, we put it in the full version paper~\cite{psiPaperFull}}\iffullversion{Due to the space limit, we put it in \cref{app:treeHeightSupport}.}
  The high-level idea is to replace $t=\log n$, so $\delta=f(t)=-t/(\log(1/2-1/t))-t=t/(1+\log t-\log(t-2))-t$.
  We show that $f(t)$ is decreasing for $t\ge 2$ by proving $f'(t)<0$ for $t\ge 2$.
  Since we have several logarithmic functions in the denominator, we computed the second and third derivatives and used a few algebraic techniques to remove them.
\end{proof}
\hide{
  \begin{proof}
    %The first part of this lemma is simple.
    Plugging in $\os\ge\log n$ to \cref{lem:sampling} gives $\epsilon\le 1$ \whp, so one subtree can have at most 3/4 of the size of the parent---the tree size shrinks by a quarter every level.
    This indicates the tree heights to be $O(\log_2 n)$ \whp.

    We now show the second part of this lemma, which is more mathematically interesting. W.l.o.g let leaf wrap $\leafwrap=4$, so that the tree has height 1 for $n\leq 4$.
    By plugging in $\epsilon=O(1)/\log n$, the tree height $h$ can be solved as $\log n+O(1)$.
    Similar to the above, here in the worst case, the children's subtree size shrinks by at least $1/2+\epsilon/4$.
    For simplicity, we let $\epsilon=4/\log n$ so $1/2+\epsilon/4=1/2+1/\log n$.
    Hence, the tree height satisfies $(1/2+1/\log n)^h=1/n$, so $h={-\log n}/{\log(1/2+1/\log n)}$.
    We will show that $\delta=h-\log n={-\log n}/{\log(1/2+1/\log n)}-\log n=O(1)$ for $n> 4$.
    \ifconference{
      This analysis is quite complicated---due to the space limit, we put it in the full version of the paper~\cite{pkdPaperFull}.
    }
    \iffullversion{
    This analysis is quite complicated---due to the space limit, we put it in the \cref{app:treeHeightSupport}.  }
    The high-level idea is to replace $t=\log n$, so $\delta=f(t)=-t/(\log(1/2-1/t))-t=t/(1+\log t-\log(t-2))-t$.
    We show that $f(t)$ is decreasing for $t\ge 2$ by proving $f'(t)<0$ for $t\ge 2$.
    Since we have multiple logarithmic functions in the denominator, we can compute the second and third derivatives and a few algebraic techniques to remove them.
  \end{proof}
}

Later, we will experimentally show that maintaining strong balancing criteria (tree height of $\log_2 n+O(1)$) is not necessary for most \kdtree{}'s use cases.
Hence, in the rest of the analysis, we will use $\os=\Theta(\log n)$ and assume the tree height as $O(\log n)$.

With these lemmas, we now show that \cref{algo:constr} is theoretically efficient in work, span, and cache complexity, if we plug in the appropriate parameters.
Recall that $M$ is the small memory size.
We will set 1) skeleton height $\levels=\epsilon\log M$ for some constant $\epsilon<1/2$;
and 2) chunk size $l=2^\levels$, so array $A$ and $B$ have size $O(2^{\levels}\times |P|/l)=O(|P|)$,
and operations on $A$ and $B$ will have $O(1)$ cost per input point on average.
We use $O(\mb{Sort}(n))=O((n/B)\log_M n)$ to refer to the best-known cache complexity of sorting $n$ keys, which is also a lower bound
for \kdtree{} construction---consider that the input points are in one dimension, then building a \kdtree{} is equivalent to sorting all points by their coordinates.
We also assume $M=\Omega(\polylog(n))$, which is true for realistic settings.

\begin{theorem}[Construction cost]\label{thm:constr}
%With $\levels=\epsilon\log M$ and $l=2^\levels$,
With the parameters specified above,
\cref{algo:constr} constructs a \ourkdtree of size $n$ in optimal $O(n\log n)$ work and $O(\mb{Sort}(n))=O((n/B)\log_M n)$ cache complexity, and has $O({M}^{\epsilon}\log_M n)$ span for constant $0<\epsilon<1/2$, all with high probability.
Here $M$ is the small-memory size and $B$ is the block size.
%, for $\os=\polylog(\log n)$ and $\levels=(\log M)/2$.
\end{theorem}

\begin{proof}
We start with the work bound.
Although the entire algorithm has several steps,
each input point is operated for $O(1)$ times in each recursive level, except for \cref{line:loopup-1,line:loopup-2}.
For these two lines, looking up the bucket id has $O(\levels)$ work.
Since the total recursive depth of \cref{algo:constr} is $O(\log n)/\levels$ \whp{},
the work is $O(\levels\cdot(\log n)/\levels)=O(\log n)$ \whp{} per input point,
leading to total $O(n\log n)$ work \whp{}.

\hide{
% We now analyze the span and I/O cost of \cref{algo:constr}.
We now analyze the span of \cref{algo:constr}.
% Again, we mainly focus on the \textsc{Sieve}() function since the other part only deals with $2^\levels\cdot\os=\sqrt{M}\log n$ samples \ziyang{should we use $\Theta(\sqrt M\log n)$?}, and builds a tree skeleton with $\levels$ levels.
The algorithm starts with sampling $2^\levels\cdot\os$ points and build a tree skeleton with $\levels$ levels.
%Based on our parameter choosing, this part fully fits in cache.
Using the standard \kdtree construction algorithm (mentioned at the beginning of \cref{sec:constr}) gives $O(\levels \log n)$ span,
%In the sieving step, each chunk has $l=2^{\levels}$ elements that are processed sequentially, and all chunks are processed in parallel.
%This gives $O(2^{\levels})$ span.
%which is dominated by the $O(M^{\epsilon}\log n)$ span for sampling.
which is dominated by the $O(2^{\levels})=O(M^{\epsilon}\log n)$ span for sampling.

We now focus on the span of \textsc{Sieve}().
There are two loop bodies, \cref{line:seq-loop-1,line:seq-loop-2}, that are executed sequentially.
The span for them is hence the same as the work analyzed above, which is $O(l\levels)$.
The column-major prefix sum on \cref{line:transpose} can be computed in $O(\log n)$ span~\cite{blelloch2010low}, and all other parts also have $O(\log n)$ span.
The total span for one level of \textsc{Sieve}() is therefore $O(l\levels+\log n)$.
Since \cref{algo:constr} have $O(\log n)/\levels$ recursive levels \whp, the span for \cref{algo:constr} is $O(l\levels+\log n)\cdot O(\log n)/\levels=O(2^\levels\log n+\log^2n/\levels)=O(M^{\epsilon}\log n)$ \whp, assuming $M^{\epsilon}>\log n$.
}

We now analyze the span of \cref{algo:constr}.
The algorithm starts with sampling $2^\levels\cdot\os$ points and building a tree skeleton with $\levels$ levels.
%Taking samples is executed sequentially, which has $O(2^{\levels})=O(M^{\epsilon}\log n)$ span.
%Since all samples fit in cache,
Taking samples and building the skeleton on them can be trivially parallelized in $O(\lambda\log n)$ span (using the plain algorithm at the beginning of \cref{sec:constr}).
%In the sieving step, each chunk has $l=2^{\levels}$ elements that are processed sequentially, and all chunks are processed in parallel.
%This gives $O(2^{\levels})$ span.
%which is dominated by the $O(M^{\epsilon}\log n)$ span for sampling.
%which is dominated by the $O(2^{\levels})=O(M^{\epsilon}\log n)$ span for sampling.
In the sieving step, each chunk has $l=2^{\levels}$ elements that are processed sequentially, and all chunks are processed in parallel.
This gives $O(2^{\levels})$ span.
The column-major prefix sum on \cref{line:transpose} can be computed in $O(\log n)$ span~\cite{blelloch2010low}, and all other parts also have $O(\log n)$ span.
The total span for one level of recursion is therefore $O(l+\log^2 n)=O(M^{\epsilon})$, assuming $M=\Omega(\mathit{polylog(n)})$.
Since \cref{algo:constr} have $O(\log n)/\levels$ recursive levels \whp{}, the span for \cref{algo:constr} is $O(M^{\epsilon}\log_M n)$ \whp.

We finally analyze the cache complexity.
Based on the parameter choosing, the samples fully fit in the cache.
In each sieving step, since $l=2^\levels=M^{\epsilon}\le \sqrt{M}$, the array $A[i][\cdot]$ and $B[i][\cdot]$ fits in cache, so the loop bodies on \cref{line:seq-loop-1,line:seq-loop-2} will access the input points in serial, incurring $O(n/B)$ block transfers.
All other parts cost $O(n/B)$ block transfers, including the column-major prefix sum on \cref{line:transpose}~\cite{blelloch2010low}.
Hence, the total cache complexity for \cref{algo:constr} is $O(n/B)$ per recursive level, multiplied by $O((\log n)/\levels)=O(\log n/\log M)=O(\log_M n)$ levels \whp, which is $O(n/B\cdot \log_M n)$.
\end{proof}

The work and cache bounds in \cref{thm:constr} are the same as sorting (modulo randomization)~\cite{aggarwal1988input} and hence optimal.
The span bound can also be optimized to $O(\log^2 n)$ \whp{}, using a similar approach in~\cite{blelloch2010low}, with the details given in the proof of the theorem below.
\hide{We still use the previous version in the implementation, because in practice, $O({M}^{\epsilon}\log_M n)$ span bound is good enough to achieve sufficient parallelism,
and the solution with stronger span bound may incur a larger constant that slows down the overall performance. }

\begin{theorem}[Improved span]\label{thm:constr-polylog}
A \ourkdtree of size $n$ can be built in optimal $O(n\log n)$ work and $O(\mb{Sort}(n))=O((n/B)\log_M n)$ cache complexity, and has $O(\log^2 n)$ span, all with high probability.
\end{theorem}

\begin{proof}
The $O(2^\levels)=O({M}^{\epsilon})$ span per recursive level is caused by the two sequential loops on \cref{line:seq-loop-1,line:seq-loop-2}.
These two loops can be parallelized by a sorting-then-merging process as in~\cite{blelloch2010low}.
The high-level idea is to first sort (instead of just count) the entries in the loop on \cref{line:seq-loop-1} based on the leaf labels.
Once sorted, we can easily get the count of the points in each leaf.
Then on \cref{line:seq-loop-2}, once the array is sorted, points can be distributed in parallel.
We refer the readers to~\cite{blelloch2010low} for more details.
The span bound for each level is $O(\log n)$~\cite{blelloch2010low,blelloch2020optimal} for the sieving step.
For the rest of the part, the span is $O(\lambda\log n)$ caused by skeleton construction.
Altogether, the span per level is $O(\lambda\log n)$, and there are $O(\log n/\lambda)$ recursion levels \whp.
Therefore, the total span is $O(\log^2 n)$ \whp.
\end{proof}

In practice we still use the previous version because $O({M}^{\epsilon}\log_M n)$ span can enable sufficient parallelism,
and the additional sorting to get the improved span may lead to performance overhead.


==> cover_page.tex <==
\twocolumn[
{\centering
	\Huge Pkd-tree: Parallel $k$d-tree with Batch Updates \\
	Revision Summary \\[.6em]
}
{\sffamily
	We provide three files in this submission:

	\medskip
	{\bf Revision.pdf}\space\space{\small The revised manuscript for the conference paper with 13 pages (excluding references).}

	\medskip
	{\sffamily\bf Cover\_letter\_and\_full\_paper.pdf}\space\space
	{\small This document contains the cover page and the full version of the paper, including the conference version as the main text, and supplementary materials in the appendix. Due to the page limit, we were not able to add all the contents required by the reviewers in the main paper, but we provided detailed experimental results and discussions in the full version of the paper. As we mentioned in the cover letter, we plan to upload the full version to ArXiV to make all results in the appendices available to the public. 

	We combine the cover letter and the full paper such that the hyperlinks in the cover letter to all sections and appendices are preserved.}

	\medskip
	{\sffamily\bf Diff.pdf}\space\space
	{\small It contains all modifications outlined in this document, as well as minor adjustments to the wording to ensure the conference version fits within 13 pages. 
	These changes are purely stylistic, and no substantive content or meaning has been altered.}
% This file highlights differences of the revised manuscript from the last submission, with the added text colored blue and the discarded text colored red and struck out. 
	% Aside from necessary changes based on the review, we made minor adjustments to the wording to ensure the document fits within 13 pages. These adjustments are purely stylistic, and no substantive content or meaning has been altered.}
	\\[.6em]
}]
\setcounter{page}{1}
We express our gratitude to the reviewers for the time and effort dedicated to the reviewing of our submitted manuscript.
% The suggestions are very helpful, and we will surely address all of them.
% Most of these comments should be easily addressed by adding more explanations and discussions or supplementing a few experimental numbers.
% However, there are a few of them that we may want to see if our shepherd thinks whether our plan or explanations are reasonable, particularly for \oref{R2O4}, \oref{R2O5}, and \oref{R3O2}.
This document summarizes the changes we made to the manuscript in response to the review comments after discussion with the reviewers.
We will keep the section, figure, and table references identical to the ones in the paper.
Due to page limits, some proposed revisions, as well as some raw data of experimental results,
are elaborated in the full version (provided as the \emph{supplementary material}).
We plan to upload the full version of the paper on arXiV to make the results publicly available.
Since two reviewers mentioned the importance of real-world datasets, we prioritize the new experiments about real-world datasets and put them into the main paper.
%\ziyang{The camera-ready length is 13 pages excluding references, should we still mention that we will include all contents within the main paper after accept? }
We also highlight the modified components in blue for easy identification.
% We express our gratitude to the reviewers for the time and effort dedicated to the reviewing of our submitted manuscript.
% The suggestions are very helpful, and we will surely address all of them.
% Most of these comments should be easily addressed by adding more explanations and discussions or supplementing a few experimental numbers.
% However, there are a few of them that we may want to see if our shepherd thinks whether our plan or explanations are reasonable, particularly for \oref{R2O4}, \oref{R2O5}, and \oref{R3O2}.
% This document summarizes the changes we made to the manuscript in response to the review comments after discussion with the reviewers.
% This document contains the cover page and the full version of the paper, including the conference version as the main text, and supplementary materials in the appendix.
% It summarizes the changes we made to the manuscript in response to the review comments after discussion with the reviewers.
% We combine the cover letter and the full paper such that the hyperlinks in the cover letter to all sections and appendices are kept. 
% Due to page limit, we were not able to add all contents required by the reviewers in the main paper, but we provided detailed experimental results and discussions in the full version of the paper.
% As we mentioned in the cover letter, we plan to upload the full version to ArXiV to make all results in the appendices available to the public.

% We will keep the section, figure, and table references identical to the ones in the paper.
% Due to page limits, some proposed revisions, as well as some raw data of experimental results,
% are elaborated in the full version (provided as the \emph{supplementary material}).
% We plan to upload the full version of the paper on arXiV to make the results publicly available.
% Since two reviewers mentioned the importance of real-world datasets, we prioritize the new experiments about real-world datasets and put them into the main paper.
% %\ziyang{The camera-ready length is 13 pages excluding references, should we still mention that we will include all contents within the main paper after accept? }
% The modified components are highlighted in blue for easy identification.
%We also summarize the reviews of every reviewer below to confirm that we understand the feedback correctly.
% We thank the reviewers for their constructive suggestions and comments.  In this letter, we summarize how we address the required and optional changes in the meta-review, as well as other revisions to address the individual comments from reviewers. We hope that these changes have addressed the reviewer's concerns. In this letter, we keep pointers to \revision{Sections}, \revision{Figures}, \revision{Tables}, and \revision{Algorithms} in the revised paper, which is attached at the end of this cover letter. We have also highlighted the modified components in a different color for easy identification. 

%In the following, we discuss each of the reviewer's comment, the solution we proposed in revision plan, as well as the changes in the revised manuscript. 
% We include the document for visual difference as the supplementary material. 
% It contains all modifications outlined here, as well as minor adjustments to the wording to ensure the conference version fits within 13 pages. 
% These changes are purely stylistic, and no substantive content or meaning has been altered.
% All modifications are highlighted in the visual difference material. 


\section*{Reviewer 1}
\begin{tcolorbox}
	\textbf{R1O1}\label{R1O1} All the experiments are restricted to dimensions $<10$ (and mostly 2 and 3) ... It would be good to have a comparison on how the proposed approach performs in higher dimensions greater than 10.\\
	\textbf{Revision Plan:} We will include a high-dimensional synthetic dataset, and a high-dimensional real-world dataset. We will also add discussions about the new experiments on the high-dimensional datasets.
\end{tcolorbox}
% Certainly. We will include more experiments for this study.
% We will include a new real-world dataset \texttt{CHEM}~\cite{fonollosa2015reservoir,wang2021fast} including 4.21M points with dimension 16.
% We can add another study regarding dimensionality vs.\ update/query performance on our synthetic datasets.
% This study may go to the full version of this paper, depending on the space we have for the revised version and the final version.
We included a new real-world dataset \texttt{CHEM}~\cite{fonollosa2015reservoir,wang2021fast} with 4.21M points and 16 dimensions in \cref{table:real-world}.
We also added an experiment on synthetic datasets in 12 dimensions.
The data generator for Varden~\cite{gan2017hardness} was not able to generate 1000M points in 12 dimensions in 24 hours.
Therefore, we present an experiment on the synthetic dataset with 100M points in 12 dimensions in \cref{table:highdimsyn} with discussions in \cref{paper:app:synthetic} in the supplementary material.
%\ifconference{in the supplementary material.}\iffullversion{in \cref{paper:app:synthetic}.}

\textbf{The new results are in \cref{table:real-world} in the main paper (for real-world datasets), and \cref{table:highdimsyn} in the full paper (for synthetic datasets).
	The discussions are highlighted in \cref{sec:exp:real-world} in the main paper and \cref{paper:app:synthetic} in the full paper. }


\section*{Reviewer 2}
\begin{tcolorbox}
	\textbf{R2O1}\label{R2O1} The authors should provide specific (real) motivating examples where the dataset scale is so huge as to necessitate parallel processing and fast processing.

	\textbf{Revision Plan:} We will add real motivating examples to show the need for parallel processing of large-scale spatial data.
\end{tcolorbox}
% Sure.  We will elaborate on this in the final version.
% For instance, the \texttt{OSM} dataset we tested has more than $10^9$ points, and even CGAL (a less efficient parallel solution) already uses about 500 seconds just to construct the index. In comparison, our solution only takes 5 seconds.
In \cref{paper:sec:intro}, we use the \texttt{OSM} as a motivating example, which contains 1.29B points with 2 dimensions.
Sequentially, it takes about 2000 seconds to build the tree using the widely-used computational geometry library \cgal{}.
%With our new parallel algorithm running on 96 cores, it only takes about 5 seconds to construct the tree.
%, while a highly parallel implementation \ourlib{} can construct the tree using about 5 seconds. 

\textbf{The revisions are highlighted in \cref{paper:sec:intro}.}

\begin{tcolorbox}
	\textbf{R2O2}\label{R2O2} How do the (state-of-the-art) parallel R-tree implementations compare with the \ourtree{} in terms of practical performance?

	\textbf{Revision Plan:} We will expand on the discussion on parallel R-trees. We will add experiments on R-tree constructions and queries.
\end{tcolorbox}
% This is a good point.
% The discussion for this question is in the last paragraph in \cref{paper:sec:related}, and we can surely elaborate on this.
% Unfortunately, we are unaware of R-tree algorithms or open-source implementations that support efficient parallel updates---we are also considering it as an interesting future work.
% This is probably not surprising, given that the main use cases for R-trees are for external memory, while the thread-level in-memory parallelism is a less relevant optimization.
% Currently, we have included the comparison to quad/octrees in the supplementary document.
% We can include a comparison to some existing in-memory R-tree implementations on construction and queries in the final full version.

We compare the \ourlib{} and an in-memory \rtree{} implementation in the Boost library~\cite{schaling2011boost}.
We note that the Boost \rtree{} only supports sequential construction and updates (insertion and deletion)\footnote{We did not find available \rtree{} implementations that support parallel batch updates.
	Therefore, we compare with the sequential \rtree{} in the widely-used Boost library.}.
Therefore, we study the speedup of \ourtree{} over their sequential version on construction and updates.
We parallelized the \knn{} and range queries for \rtree{} for comparison.

We present the comparison with \rtree{s} and \zdtree{s} (a variant of quad/octree) in \cref{table:app_rtree_zdtree} in \cref{app:rtree} in the supplementary material.
%We combine the comparison with \rtree{s} and the comparison with \zdtree{s} (a variant of quad/octree) in the full version (supplementary material).
The performance mainly indicates the difference between data structures.
We note that the \rtree{} itself also supports more general functionalities than \kdtree{s}, such as range queries with arbitrary shapes, spatial overlap/intersection queries, handling non-point and high-dimensional objects, and may not be specifically optimized for \knn{} or range queries.
In general, our \ourtree{} using 96 cores is 90--115$\times$ faster than the sequential \rtree{} in construction, 30--580$\times$ faster in batch insertions, and 133--2259$\times$ faster in deletion.
For \knn{} queries, all three implementations (\ourtree{}, \zdtree{} and Boost \rtree{}) can run in parallel.
The \ourtree{} is about 10$\times$ faster than the \rtree{}, and about 2$\times$ faster than the \zdtree{}.
More detailed discussions are available in \cref{app:rtree}.

\textbf{The new results are in \cref{table:app_rtree_zdtree} in the supplementary material. The discussions are highlighted in \cref{app:rtree} in the supplementary material.}

\begin{tcolorbox}
	\textbf{R2O3}\label{R2O3} In preliminaries, about the cache model used: ``assuming the \emph{optimal offline} cache replacement policy''. ... There should definitely be more explanation and justification here, and if my fear is valid, the implementation should use a feasible eviction policy like MRU, LRU, etc as this could draw a completely different picture in the experiments.

	\textbf{Revision Plan:} We will explain the model in more detail in the preliminary. We will also clarify that the optimal replacement policy is not used in implementation.
\end{tcolorbox}
% Thanks for the clarification questions.
% For the theoretical analysis, we use the ideal-cache model, proposed in~\cite{Frigo99},
% which is a widely-used model to analyze the cache complexity for in-memory algorithms in theory.
% %The model has nothing to do with how the algorithm is implemented (we released our code in \cite{pkdCode}).
% The ideal-cache model assumes the optimal offline cache replacement policy for simplicity,
% and the original paper~\cite{Frigo99} has proved that the number of cache misses in practical policies can be off by at most a constant factor than the optimal policy (e.g., a factor of 2 for LRU).
% In other words, the \emph{asymptotic} cost bounds in big-O provided in our paper also hold for LRU.
% %More practically, they have negligible differences. 
% We can surely elaborate on this more when defining this model and summarize the theoretical results in~\cite{Frigo99} to avoid possible confusion.
We added more discussion in \cref{paper:sec:prelim} to clarify the definition of the model. We also clarified that one cannot guarantee to use an optimal strategy in reality, and thus the assumption is only used for simplicity for theoretical analysis.

\textbf{The revisions are highlighted in \cref{sec:prelim} in the main paper. }

\begin{tcolorbox}
	\textbf{R2O4}\label{R2O4} In the experiments of \cref{paper:tab:introTable}, the range queries report $10^4$ to $10^6$ records, which is huge and unpractical. Please (A) explain why it is meaningful, or (B) unless there is a very strong justification for (A), experiments should be provided also for much more selective queries too.

	\textbf{Revision Plan:} We will use Figure 5 to discuss more.
\end{tcolorbox}
% Thanks for the comments.
% We have provided experiments on range count and range report queries on the full spectrum of output size (from 1 to $10^6$) in \cref{paper:fig:rquery}.
% We note that range count and range report queries are widely used and have many applications with various output sizes.
% For instance, we are aware of some dynamic programming applications using large-range queries (e.g.,~\cite{shen2022many,gu2023parallel}).
% In \cref{paper:tab:introTable}, we choose to report range queries with larger sizes since they take longer time and are more adversarial test cases than small range queries.
% %We pick larger range queries to report since the running times are longer and have smaller variance (see \cref{paper:fig:rquery} as a reference).
% We can, of course, use smaller ones in \cref{paper:tab:introTable} instead if the reviewer thinks it necessary.
As discussed with the reviewer, we will keep \cref{fig:rquery} to illustrate the query performance with varying output sizes.
%The \cref{paper:fig:rquery} has shown the performance of range queries with different output sizes, from 1 to $10^6$.
%We explained in the caption of \cref{table:summary} why we choose a large query range in the summary table. 
We also added more details in \cref{sec:exp:operation} to discuss results in \cref{fig:rquery}.

\textbf{The revisions are highlighted in the caption of \cref{table:summary} and \cref{sec:exp:operation} paragraph ``Range Queries''.}

\begin{tcolorbox}
	\textbf{R2O5}\label{R2O5}
	The paper uses $\alpha = 0.3$ by default, which means that a subtree’s size can be 4 times shorter/taller than its sibling. ... the authors should explain how frequent and how extensive the partial reconstruct/rebalancing works are to convince the reader that rebalancing is actually happening a lot in the experiments but performance is smooth because update handling is very efficient (as opposed to the paper presenting good performance because in effect the updates are suppressed by $\alpha$ and rarely require heavy reconstruction effort).

	\textbf{Revision Plan:} We will show Pkd-tree’s performance with original $\alpha$, $\alpha=0.1$, and $\alpha = 0.03$. We will also measure the total number of reconstructed nodes in batch updates.
\end{tcolorbox}
Based on the discussion with the reviewer, we evaluated the performance of \ourlib{} on batch update with $\alpha=\{0.03, 0.1, 0.3\}$ in \cref{table:3inba} in the supplementary material. The discussions are in \cref{app:inbaratios}.
In the original discussion, the plan was to use different $\alpha$ for all results in \cref{table:summary}.
We note that in \cref{table:summary}, the construction time is not affected by the value of $\alpha$ (there is no rebuild in construction).
Also, in \cref{paper:table:summary}, the queries were directly performed on the tree after construction, and therefore is also not affected by the value of $\alpha$.
Therefore, in the final revision, we only include the running time for batch insertions and batch deletions in \cref{table:3inba} in the supplementary material.
In addition to \ourtree{} with three values of $\alpha$, we also include the numbers for \logtree{}, \bhltree{} and \cgal{} in the same table for comparison.

To study the query performance under different values of $\alpha$, it is necessary to run a large number of updates before the query such that the imbalance ratio will significantly affect the shape of the tree. Such experiments are essentially the same as \cref{fig:inbaRatio} in our original paper. Based on the discussion with the reviewer, we also include the number of nodes involved in reconstructions in this figure in our revised paper.
Discussions are included in \cref{paper:sec:balancingParameterRevisted}.

%We also extended the experiments described in \cref{paper:sec:balancingParameterRevisted} to include the sum of the rebuild tree sizes during batch updates for various values of $\alpha$, as detailed in \cref{app:rebuild}. 

\textbf{\boldmath The result of the running time under $\alpha=\{0.03, 0.1, 0.3\}$ is in \cref{table:3inba} in the supplementary material,
	and discussions are in \cref{app:inbaratios} in the supplementary material.
	The experiments on the number of reconstructed nodes under different values of $\alpha$ are integrated in \cref{fig:inbaRatio}, and discussions are highlighted in \cref{paper:sec:balancingParameterRevisted}.
	\unboldmath}

\begin{tcolorbox}
	\textbf{R2O6}\label{R2O6} In the experimental setup ``We ran each experiment 4 times and report the average of the last 3 runs''. Why exactly do you do this and why is it fair? Is this the norm in how experiments in related work are run? Does this give your method an advantage? Please show (even only in the response letter) performance in a few indicative settings where the experiments are ran only once.

	\textbf{Revision Plan:} We will briefly explain the reason in the paper.
\end{tcolorbox}
% \input{run_once_table.tex}
\hide{ Yes. This is a common practice for testing parallel algorithms to run a warm-up round first.
	We observed that in the open-source code of the ParGeo library that we tested as a baseline,
	the experimental setting is also to run four times and discard the first warm-up round.
	The other baseline \zdtree{} (as part of the PBBS library~\cite{anderson2022problem}) first runs one or multiple warm-up rounds for at least one second and then reports the running time of the subsequent rounds.
	%In fact, the related work~\cite{blelloch2022parallel,wang2022pargeo} is all tested in this manner (as we can tell from the open-source testing code). 
	%Similar settings are also used in some parallel benchmarks. 
	%For example, in the open-source library Problem-Based Benchmark Suite~\cite{anderson2022problem}, which also includes the 

	The reason for doing this is due to the cache state---the running time can depend on what was in the cache before the program/operation runs.
	% By excluding the first warm-up round, we can guarantee that the timed runs always see the same cache configuration, thus leading to a performance with smaller variance (i.e., excluding the variation on what was run previously).
	By excluding the first warm-up round, we ensure that all timed runs start with the same cache configuration, thus leading to a performance with a smaller variance (i.e., excluding the variation on what was run previously).
	% By excluding the first warm-up round, we ensure that all timed runs start with the same cache configuration. This reduces performance variability, i.e., excluding the variation on what was run previously, which results in more consistent and reliable timing results.

	To help the reviewer better understand the above claim, we run some experiments in \cref{tab:seq} (in this document) to demonstrate it.
	The running time of the first run (\#0) has a much larger variance, depending on the previous operation(s), while the last three are much stabler.
	% For example, we first compare the first two entries in \cref{tab:seq}.
	% When the batch insert happens directly after the construction,
	For example, by comparing the first two entries in \cref{tab:seq}, where the batch insert happens directly after the construction,
	the first run of the batch insertion can take 0.174s, while the next three runs all take about 0.100--0.110s.
	Instead, if we first run a construction, then insert the batch, delete it, and insert it back again, all four runs of the last insertion take a similar time, around 0.100--0.110s.
	%Particularly for the same insertion operation (Line 1 and Line 3 in \cref{tab:seq}), the first run can be drastically different, depending on the previous operations (and subsequent cache states).
	Including the first run actually adds the variance caused by the previous operation, while excluding the first run diminishes it.
	% While it seems that this experiment configuration should have been applied to all settings, it is particularly sensitive to the parallel algorithm experiments since parallel algorithms run faster, and such variances can be exaggerated.
	Although this experimental configuration should ideally be applied to all settings, it is significant for the parallel algorithm experiments, since parallel algorithms run faster, making them more prone to exaggerated performance variances.
	The third and fourth entries show the running time of the initial run for the \knn{} and the range query tested in \cref{paper:tab:introTable} in the original paper.
	We can see that the first run is not always much slower.
	Therefore, to report more consistent results, we always exclude the first run.
	%This effect is similar for other tested algorithms, and as mentioned, the original papers of the baseline algorithms~\cite{blelloch2022parallel,wang2022pargeo} are also tested in this manner. 
	%Almost all tables and figures in the paper contains running times close to or smaller than 100 milliseconds, and running times in such scales necessitate such a configuration. 
}
As we have discussed in our previous revision plan, this is mainly used to keep the cache configuration identical before every experiment.
We clarified more about this setting in \cref{paper:sec:exp}.

\textbf{The revision is highlighted in \cref{paper:sec:exp}, paragraph ``Setup''.}

\begin{tcolorbox}
	\textbf{R2O7}\label{R2O7} Please provide an experiment where the dataset is Varden but the NN queries are Uniform.

	\textbf{Revision Plan:} We will add some out-of-distribution queries.
\end{tcolorbox}
% This is a good point.
% %We indeed tested some out-of-distribution queries before we submitted the paper and the performance is similar.
% We will include these experiments in the paper, likely in the supplementary materials.
% We included the experiment results where the tree contains points from \varden{} but the query points
We included the result for the experiment suggested by the reviewer in \cref{app:ood}.
We also include the experiment where the tree contains points from \uniform{} but the query points are from \varden{}.

\textbf{New experimental results are in \cref{table:ood} with discussions in \cref{app:ood}, both in the supplementary material.}

\begin{tcolorbox}
	\textbf{R2O8}\label{R2O8} What algorithm did the paper use for NN processing? Is there any particular reason for that choice? To my knowledge there is no single standard algorithm. There are several options like depth first, best first, etc. Which option was used and is there any particular reason for that choice?
\end{tcolorbox}
% We use the standard depth-first search algorithm for NN processing, which traverses the subtree that the query point resides (not necessarily contained in the subspace of the subtree)\footnote{For every query point $q$, when it first visits a non-leaf node $T$, if $q$ is to the left of the splitter in $T$, it will visit the $T.lc$ then, and vice versa.
% 	After the recursion returns, we can prune the visit to the other child of $T$ by the distance between $q$ and the splitter in $T$.
% 	When $q$ reaches to a leaf node, we will traverse all points stored within the leaf in serial and add them to the candidate container correspondingly.
% }.
%We choose this since it is the common practice in many geometric applications such as in computer graphics.
% This algorithm is widely used in many geometric applications such as in computer graphics.
As briefly mentioned in the revision plan, we use the standard depth-first search algorithm,
which first traverses the subtree that the query point resides (not necessarily contained in the subspace of the subtree).
For example, when searching the query point $q$ in a non-leaf subtree $T$, if $q$ is to the left of the splitter of $T$, it will visit the $T.lc$ first, and vice versa.
After the recursion returns, we can prune the visit to the other child of $T$ by the distance between $q$ and the splitter in $T$.
When $q$ reaches to a leaf node, we will traverse all points stored within the leaf in serial and add them to the candidate container correspondingly.
%We choose this since it is the common practice in many geometric applications such as in computer graphics.
We add this description about the NN query and range count/report algorithms in \cref{paper:sec:impl}.

\textbf{The revision is highlighted in \cref{paper:sec:impl}}.

\begin{tcolorbox}
	\textbf{R2O9}\label{R2O9} In Section 6.2 I believe no experiment is shown for Range/Range-count queries and Deletions. ... I found the section on real datasets small (which is fine, as it is the authors prerogative how to allocate space) but at least each aspect of the work should be evaluated on them too.
	\textbf{Revision Plan:} We will add range queries and deletions in our experiments on real-world datasets.
\end{tcolorbox}
% Thanks for the suggestions.
% We will add these experiments to the final version.
% Regarding deletion operations, we will use the sliding-window setting on the \texttt{OSM} dataset.
We added range report queries for all real-world datasets. The results are presented in \cref{paper:table:real-world} and a discussion is presented in \cref{paper:sec:exp:real-world}, paragraph ``Tree Construction, \knn{} and Range Report''.

To measure the performance of batch deletion, we simulate a sliding-window setting on the \texttt{OSM} dataset. Recall that the dataset contains 2 dimensional points with timestamps from 2014 to 2023.
We start with building a tree of the data in 2014.
We then insert the batch for each year into the tree, and delete the batch of five years ago if applicable.
After the update of each year, we perform 10-NN queries.
We compare the performance among all baseline algorithms.
The results are presented in \cref{paper:fig:osm-batch}, and a discussion is in \cref{sec:exp:real-world}, paragraph ``Dynamic Updates''.
%The batch deletion is measured using the sliding-window setting on the \texttt{OSM} dataset, and the result is demonstrated in \cref{paper:fig:osm-batch}.

\textbf{The new experimental results about range queries are in \cref{paper:table:real-world}. The new experimental results about deletions are presented in \cref{fig:osm-batch}. The discussions for these new results are highlighted in \cref{sec:exp:real-world}. }

\begin{tcolorbox}
	\textbf{R2O10}\label{R2O10} Maybe the authors should add~\cite{blelloch2022parallel} to the summary in Table 5.
\end{tcolorbox}
% We did not include it because the \zdtree{} is a quad/octree structure, while \cref{paper:tab:related} summarizes all works related to \kdtree{s}.
% Hence, it does not seem to be a good fit (e.g., quad/octree does not rebalance).
% However, we can add it to the table if the reviewer recommends.
%However, we will elaborate this more in the discussion and distinguish their differences.
Based on the discussion with the reviewer, we keep \cref{paper:tab:related} as is, and compare to~\cite{blelloch2022parallel} (\zdtree{}) in \cref{app:zdtree} in the supplementary material.

\section*{Reviewer 3}
\begin{tcolorbox}
	\textbf{R3O1}\label{R3O1} The parallel construction needs to compare with the state-of-the-art in data management community, i.e., \cite{reif2022scalable}. I expect comparing and contrasting with the construction process. It is unfortunate that the kd-tree in \cite{reif2022scalable} does not appear to have an open source implementation, so conceptual comparison is needed.
\end{tcolorbox}
% Sure.  We will add more discussions as we mentioned in \oref{R2O2}.
We have added discussions with more details to compare with parallel construction algorithms for static \kdtree{s} in \cref{paper:sec:related},
including~\cite{brown2014building,cao2020improved, yamasaki2018parallelizing, reif2022scalable, al2000parallel,hunt2006fast, shevtsov2007highly, choi2010parallel}.

\textbf{The revision is highlighted in \cref{sec:related}.}

\begin{tcolorbox}
	\textbf{R3O2}\label{R3O2}
	The Cache Efficiency experiments need to report more hardware performance counter numbers.
	The authors duly reported the cache misses numbers which do coincide with the performance numbers.
	First and foremost, I want the authors to investigate the IPC numbers to determine whether the range queries are memory or compute bound ... Next, the authors should also report the cache reference count, branch count and branch prediction misses. This will shed more light on data level and instruction level locality of the Pkdtree.

	\textbf{Revision Plan:} We will expand our cache-performance analysis, including the IPC, cache reference count, branch count, and branch prediction misses, to explore the trade-offs between memory usage and computational costs of the Pkd-tree. In addition to benchmarking the memory bandwidth for tree construction, cache-performance analysis will involve the profiling of hardware counters on range queries, especially on real-world datasets.
\end{tcolorbox}
\hide{ This is an interesting observation.
	We are happy to include IPC numbers as well as other mentioned statistics about cache and branch in the final version of this paper as a reference.

	%On the other hand, we note that it is not an ``coincidence'' that the reduced number of cache misses and the improved running time are similar.
	We thank the reviewer for asking about our algorithm's performance gain and the correlation with reduced cache misses.
	We believe that the consistency of the reduced number of cache misses and the improved running time is not just a ``coincidence''.
	%but indeed because our algorithm is memory-bottlenecked. 
	% This is indeed because our kd-tree construction and update algorithms, similar to most parallel in-memory algorithms in this flavor, are memory bottlenecked.
	This is because our kd-tree construction and update algorithms, like most parallel in-memory algorithms of this type, are bottlenecked by the memory bandwidth.
	As an example, the reported number of cache misses in our 1000M-3D-V in \cref{paper:fig:technique} indicates that our construction algorithm uses over 80\% of the memory bandwidth of this testing machine\footnote{We apologize that we did not provide the raw data in the paper but only the relative ratios.  We will include the raw data in our final version so the readers can compute this on their own.}. %is $6.244\times 10^9$, which indicates a 84GB/sec read/write throughput, 
	We also verify this using the Intel\textregistered{} VTune profiler.
	On our machine with a peak memory bandwidth of 443.78 GB/s, our \ourtree{} algorithms have a 327--421 GB/s usage of bandwidth in many stages during the construction and update.
	This indicates that our kd-tree construction and update algorithms are memory bottlenecked, and optimizing the cache complexity almost linearly contributes the performance.
	Therefore, the reduced cache misses and improved running time are highly correlated.
	%We intended to explain this causal relationship in \cref{paper:sec:tech:analysis}, but apparently did not provide sufficient details, particularly the raw numbers (we only gave the relative ratios) in the paper for the audience to follow our logic fully.
	We apologize for any confusion here and will add the details for this discussion in the final version of this paper.
}

We added a discussion on the usage of memory bandwidth in construction and updates, which indicates that construction and updates are memory-bottlenecked, and directly benefit from the improvement of cache efficiency.
We also tested the number of instructions, cycles, IPC, cache reference count, cache misses, number of branches, number of branch misses, for range queries on the real-world datasets.
We first present the result for our algorithm and all baselines in \cref{table:appendix:perf-hardware-full} in this \emph{cover page}.

Based on the discussion with the reviewer, we understand that the main goal of studying these hardware performance counter numbers is to investigate the impact of not storing bounding boxes on query performance.
When we compare our \ourtree{} with baselines, we observe that numerous factors can influence these hardware statistics.
These include but are not limited to: 1) different data structures and their layouts, 2) the implementations of query algorithms, 3) parallelism and scalability of each implementation, and 4) whether bounding boxes are stored or not, which is the focus of this study.
Consequently, directly comparing these numbers and drawing the relation to point 4) yields inconclusive results, as the other factors significantly contribute to the differences.

To better study the problem and eliminate other irrelevant factors, we implemented another version of our \ourtree{} that stores bounding boxes in the tree nodes.
We refer to this as \oursbb{} in \cref{table:appendix:perf-hardware-full} and also in the paper.
We test all the hardware performance counters and running time for \ourtree{} and \oursbb{}, shown in \cref{table:perf-mix}.
In this table, we also report the number of tree nodes accessed by \oursbb{} and \ourtree{} for comparison.
By comparing \ourtree{} and \oursbb{} we can observe the impact of storing bounding boxes directly.
Recall that storing the exact bounding boxes in each tree node will enable more accurate information to prune subtrees in range queries.
This benefit is more significant in high dimensions (a similar conclusion is reflected in our discussions in \cref{sec:exp:operation}).
On all datasets with high dimensions (\texttt{HT}, \texttt{HH}, \texttt{CHEM}), indeed \oursbb{} visits much fewer nodes than \ourtree{}.
Due to visiting fewer nodes in the tree, \oursbb{} also has a higher IPC, a smaller number of cache references, as well as lower running time.
For the three datasets in two or three dimensions (\texttt{GL}, \texttt{CM}, \texttt{OSM}), the effectiveness of bounding boxes is not as significant as in high dimensions.
In this case, \ourtree{} and \oursbb{} visited a very similar number of tree nodes.
On two of the datasets \texttt{CM} and \texttt{OSM}, \ourtree{} (without bounding box) even achieves lower time in query due to the benefit of a smaller memory footprint.

\textbf{The new results and discussions are presented in \cref{table:perf-mix} and \cref{sec:exp:cacheMemory}, paragraph ``Study of the Impact of Bounding Boxes'' in the main paper.
	Full results on \ourtree{} and \oursbb{} are included in \cref{table:appendix:perf-hardware} in the supplementary material.
	The experimental results about all baselines are presented in \cref{table:appendix:perf-hardware-full} in the cover letter.
}
%\ziyang{Did we benchmark the ``memory bandwidth''? Like the one in revision plan?}
%\yihan{We should add the discussion about reaching machine bandwidth in the previous revision plan.}

%We also measure above metrics for the range report queries on real-world datasets in \cref{xxx} in order to show the trade-off between memory usage and computation for \ourlib{}.



\begin{tcolorbox}
	\textbf{R3O3}\label{R3O3}
	Ideally, I would expect the opposite, with a greater emphasis on results from the real-world datasets. Last but not least, Table 4 should also include the range query results for the real-world datasets.

	\textbf{Revision Plan:} As mentioned in R1O1 and R2O9, we will add range queries and deletions in our experiments on real-world datasets. We will also add one high-dimensional real-world dataset. We will add more emphasis and discussions on real-world datasets in the experiment.
\end{tcolorbox}
% Thanks for the suggestions.
We included the range report queries and deletions for all real-world datasets in \cref{paper:table:real-world}.
We also added a high-dimensional real-world dataset for testing.
% We are happy to add more experiments and discussions to \cref{paper:table:real-world} for the real-world datasets, as we discussed in \oref{R2O9}.

\textbf{The new results are in \cref{paper:table:real-world} with discussions in \cref{sec:exp:real-world}.}


% \section*{Other Modifications Promised in the Rebuttal}


% ∙\bullet \hl{R3O3/R4O3/R1W4: Explain the choice of parameter τ\tau.}

% ∙\bullet \hl{R1W2: Evaluate hash bags}

% Note that both our algorithm and GBBS use the BGSS algorithm and perform the same computation in each round. We compare our plain version (i.e., disabling VGC) with GBBS to evaluate the improvement from hash bags, because the major difference between them is the use of hash bags.\\
% $\bullet$ \hl{R1D3: Explain the reason for different breakdown patterns.}
%
% $\bullet$ \hl{R1W2: Add more related works in data-base field and evaluate hash bags}
%
% We add XXX papers.

% \clearpage
% \pagenumbering{arabic}


\input{appendix-perf-hardware-table-full.tex}

\hide{


	Thanks for the suggestion. We understand the necessity of the comparison with \rtree{}.
	However, to the best of our knowledge,
	there is currently no available academia \rtree{} implementation that achieves parallelism on the thread level meanwhile supporting batch dynamic operations.
	As we mentioned in \cref{paper:sec:related}, existing works on parallel \rtree{} are either focusing on the GPU side\cite{you2013parallel,prasad2015gpu,luo2012parallel},
	or provide no implementation~\cite{kamel1992parallel,brinkhoff1996parallel,qi2020packing,achakeev2012sort}.

	In the full version of our paper (the supplementary material), we compare the time for tree construction and \knn{} query between \ourlib{} and the \zdtree{}\cite{blelloch2022parallel},
	which is analogous to the R-tree variant proposed in \cite{qi2020packing}.
	\ourlib{} is faster on all tests performed.
	The construction of the \zdtree{} firstly sorts input points based on their Morton value, then builds two sub-trees in parallel.
	The \zdtree{} supports batch update as well; unfortunately, after the confirmation with the authors, we certify that their implementation for batch update has correctness issues. Hence, we omit the corresponding tests.




	Range queries with large-scale records are better for pressure tests.
	We report them in the \cref{paper:tab:introTable} and \cref{paper:table:summary} in order to show the query performance of all baselines under extreme conditions.

	We have compared the range query performance with smaller record size, i.e., between 0 to 100, and illustrated the results in the \cref{paper:fig:rquery},
	where \ourlib{} shows the best performance in general.




	Repetitively running one experiment several times and reporting the median/average of the last times is a common trick used in related works, such as .
	This trick is mainly used to ensure the initial machine state for every experiment is almost identical, especially for those experiments requiring high parallelism.

	Below we show the running time for tests in \cref{paper:tab:introTable} that run only once: \ziyang{add run only once}


	\yan{remain to be checked after the exp data.}
	We select $\alpha=0.3$ for two considerations: 1) to reduce the number of rebuilds so as to improve the update performance while not sacrificing much query performance compared with settings with $\alpha> 0.3$, and 2) the increased cost for partial rebuilding is not high for settings with $\alpha<0.3$.

	To better illustrate the proportion between the sieving and rebuilding during the batch update, we could measure the number of rebuilds and the corresponding rebuilt tree size versus the different values of $\alpha$.
	Directly measuring the time for rebuilds is not easy, as they are performed in parallel. One possible solution is to measure the time for sieving, i.e., set $\alpha=0.5$, and subtract the result from the time with $\alpha=0.3$ to obtain an estimation for the rebuild time.


	since the query algorithms are based on different data structures, it is hard to draw general conclusion from them. For example, \cgal{} involves much more branches than others, and it also has more instructions. Therefore, the low IPC may be due to the additional instructions to verify certain conditions, \ziyang{e.g., handling of exception, logging, etc, } rather than the use of bounding boxes.

}

\renewcommand{\thetable}{\arabic{table}}
\setcounter{table}{0}



==> intro-table.tex <==
% Table generated by Excel2LaTeX from sheet 'Intro table'
\begin{table*}[htbp]
	\centering
	\small
	\setlength\tabcolsep{6pt} % column width
	\renewcommand{\arraystretch}{0.8} % row width

	% Table generated by Excel2LaTeX from sheet '1e9 Intro table'
	\begin{tabular}{cc|c|cccc|cccc|c|c}
		\toprule
		\textbf{Benchmark}                    & \multirow{2}[2]{*}{\textbf{Baselines}} & \multirow{2}[2]{*}{\textbf{Build}} & \multicolumn{4}{c|}{\textbf{Batch Insert}} & \multicolumn{4}{c|}{\textbf{Batch Delete}} & \textbf{10-NN }  & \textbf{Range Report}                                                                                                                                 \\
		\textbf{\boldmath($10^9$-2D)\unboldmath}                  &                                        &                                    & \textbf{0.01\%}                            & \textbf{0.1\%}                             & \textbf{1\%}     & \textbf{10\%}         & \textbf{0.01\%}  & \textbf{0.1\%}   & \textbf{1\%}     & \textbf{10\%}    & \textbf{\boldmath$10^7$ \unboldmath queries} & \textbf{\boldmath$10^4$ \unboldmath queries} \\
		\midrule
		\multirow{4}[2]{*}{\textbf{\uniform}} & Ours                                   & \underline{3.15}                   & \underline{.004}                           & \underline{.020}                           & \underline{.104} & \underline{.495}      & \underline{.004} & \underline{.022} & \underline{.121} & \underline{.526} & \underline{.381}        & \underline{.391}        \\
		                                      & \logtree                               & 37.9                               & .008                                       & .059                                       & 2.16             & 30.7                  & .436             & .168             & .396             & 3.01             & 2.96                    & 2.62                    \\
		                                      & \bhltree                               & 31.7                               & 31.0                                       & 31.2                                       & 31.4             & 39.9                  & 30.8             & 31.1             & 30.9             & 30.6             & .487                    & 2.06                    \\
		                                      & \cgal                                  & 1147                               & 1614                                       & 1562                                       & 1631             & 1660                  & .400             & 3.89             & 41.2             & 427              & 1.04                    & 311                     \\
		\midrule
		\multirow{4}[2]{*}{\textbf{\varden}}  & Ours                                   & \underline{3.66}                   & \underline{.002}                           & \underline{.007}                           & \underline{.055} & \underline{.473}      & \underline{.002} & \underline{.006} & \underline{.049} & \underline{.477} & \underline{.172}        & \underline{.382}        \\
		                                      & \logtree                               & 34.2                               & .008                                       & .057                                       & 2.01             & 28.0                  & .799             & .848             & 1.06             & 3.47             & 2.05                    & 2.63                    \\
		                                      & \bhltree                               & 30.2                               & 29.1                                       & 29.2                                       & 29.4             & 37.3                  & 29.3             & 29.2             & 29.0             & 28.0             & .239                    & 1.95                    \\
		                                      & \cgal                                  & 429                                & 867                                        & 867                                        & 849              & 836                   & .113             & 1.06             & 13.0             & 153              & .511                    & 296                     \\
		\bottomrule
	\end{tabular}%


	% Table generated by Excel2LaTeX from sheet '1e9 Intro table'
	% \begin{tabular}{c|cccc|cccc}
	% 	\toprule
	% 	                                   & \multicolumn{4}{c|}{\uniform} & \multicolumn{4}{c}{\varden}                                                                                                                  \\
	% 	\textbf{Operation}                 & \textbf{Ours}                 & \textbf{\logtree}           & \textbf{\bhltree} & \textbf{\cgal} & \textbf{Ours}    & \textbf{\logtree} & \textbf{\bhltree} & \textbf{\cgal} \\
	% 	\midrule
	% 	Build (Dataset Size = 1000M)       & \underline{3.15}              & 37.9                        & 31.7              & 1147           & \underline{3.66} & 34.2              & 30.2              & 429            \\
	% 	Batch Insert (Batch Size = 10M)    & \underline{.104}              & 2.16                        & 31.4              & 1660           & \underline{.055} & 2.01              & 29.4              & 849            \\
	% 	Batch Delete (Batch Size = 10M)    & \underline{.121}              & .396                        & 30.9              & 41.2           & \underline{.049} & 1.06              & 29.0              & 13.0           \\
	% 	10 Nearest Neighbor for 10M Points & \underline{.381}              & 2.96                        & .487              & 1.04           & \underline{.172} & 2.05              & .242              & .511           \\
	% 	Range Query ($10^4$ queries)       & \underline{.391}              & 2.62                        & 2.06              & 311            & \underline{.382} & 2.63              & 1.95              & 296            \\
	% 	\bottomrule
	% \end{tabular}%
	\vspace{.2em}
	\caption{\textbf{Running time (in seconds) for \ourtree{} and other baselines on $10^9$ points in 2 dimensions. Lower is better.} \normalfont
		``\logtree'': the parallel \kdtree using logarithmic method from the \pargeo{} library~\cite{wang2022pargeo}. 
        ``\bhltree'': the single parallel \kdtree from \pargeo{} library~\cite{wang2022pargeo}.
		%``\cgal'' is \edit{the \kdtree{} from the geometry library~\cite{cgal51}}.
        ``\cgal'': the \kdtree{} from the \cgal{} library~\cite{cgal51}.        
        ``Varden'': a skewed distribution from~\cite{gan2017hardness}.
		``10-NN'': 10-nearest-neighbor queries on $10^7$ points.
		``Range report'': orthogonal range report queries on $10^4$ rectangles, with output sizes in $10^4$--$10^6$.
		%More details are given in \cref{sec:exp}. %``10-NN'': 10-nearest-neighbor query for all points in parallel.
		%The unit of time is second and the best performance is underlined.
		Experiments are run on a 96-core machine. More details are in \cref{sec:exp}.
		The fastest time for each test is underlined. 
		\vspace{-1em}	}
	\label{tab:introTable}%
\end{table*}%




==> macro.tex <==
%%%%%%%%%%%%%%%%%%%%
% FORMAT
%%%%%%%%%%%%%%%%%%%%

\definecolor{dpcol}{RGB}{0,160,240}
\newcommand{\guy}[1]{
  \begin{quote} \color{green}\bf Guy: #1
\end{quote}}
\newcommand{\yan}[1]{{\color{violet}{\bf Yan:} #1}}
\newcommand{\yihan}[1]{{\color{blue}{\bf Yihan:} #1}}
\newcommand{\xiaojun}[1]{{\color{blue}{\bf Xiaojun:} #1}}
\newcommand{\zheqi}[1]{{\color{dpcol}{\bf Zheqi:} #1}}
\newcommand{\zijin}[1]{{\color{cyan}{\bf Zijin:} #1}}
\newcommand{\ziyang}[1]{{\color{blue}{\bf Ziyang:} #1}}
\newcommand{\laxman}[1]{{\color{purple}{\bf Laxman:} #1}}
\newcommand{\julian}[1]{{\color{purple}{\bf Julian:} #1}}
\newcommand{\jeremy}[1]{{\color{purple}{\bf Jeremy:} #1}}
\newcommand{\phil}[1]{{\color{blue} {\bf Phil:} #1}}
\newcommand{\charlie}[1]{{\color{red}{\bf Charlie:} #1}}
\newcommand{\Naama}[1]{{\color{magenta}{\textbf{Naama: }#1}}}
\newcommand{\iterative}{iterative}
\newcommand{\alert}[1]{{\color{red} \textbf{[[#1]]}}}
\newcommand{\red}[1]{{\color{red} {\bf Need to be rewritten:} #1}}
\newcommand{\idepth}[1]{D(#1)}
\newcommand{\iwork}[1]{A(#1)}
\newcommand{\mb}[1]{{\mbox{\emph{#1}}}}
\newcommand{\smb}[1]{{\scriptsize \mbox{\emph{#1}}}}
\newcommand{\mf}[1]{{\mbox{\sc{#1}}}}

% \newcommand{\edit}[1]{{#1}}
\newcommand{\edit}[1]{{\color{blue}{}#1}}
% CommentStyle
\newcommand\mycommfont[1]{\textit{\textcolor{blue}{#1}}}
%\definecolor{commentgreen}{RGB}{0,128,0}
%\newcommand\mycommfont[1]{\textit{\textcolor{commentgreen}{#1}}}
% \SetCommentSty{mycommfont}
%    kdtree:

\newcommand{\kdtree}{$k$d-tree\xspace}
\newcommand{\kdtreeS}{$k$d-trees\xspace}
%\newcommand{\zdtree}{zd-tree\xspace}
%\newcommand{\ourlib}{OURLIB}
\newcommand{\ourtree}{\mbox{\textsf{Pkd-tree}}\xspace}
\newcommand{\bhltree}{\mbox{\textsf{BHL-tree}}\xspace}
\newcommand{\logtree}{\mbox{\textsf{Log-tree}}\xspace}
\newcommand{\pargeo}{\textsf{ParGeo}\xspace}
\newcommand{\zdtree}{\textsf{Zd-tree}\xspace}
\newcommand{\rtree}{\textsf{R-tree}\xspace}
\newcommand{\cgal}{\textsf{CGAL}\xspace}
\newcommand{\ourlib}{\textsf{Pkd-tree}\xspace}
\newcommand{\balpara}{\alpha}
\newcommand{\varden}{\texttt{Varden}\xspace}
\newcommand{\uniform}{\texttt{Uniform}\xspace}

\newcommand{\pleft}{\prec}
\newcommand{\lson}{\ell}
\newcommand{\rson}{\textit{r}}

\newcommand{\createLeaf}{\textsc{CreateLeafNode}}
\newcommand{\createInterior}{\textsc{CreateInteriorNode}}
\newcommand{\createBucket}{\textsc{CreateBucketNode}}
\newcommand{\buildTreeSkeleton}{\textsc{BuildTreeSkeleton}}
\newcommand{\seievePoints}{\textsc{SievePoint}}
\newcommand{\build}{\textsc{BuildTree}}
\newcommand{\PickDim}{\textsc{PickSplitDimension}}
\newcommand{\fetchTreeSkeleton}{\textsc{FetchTreeSkeleton}}
\newcommand{\batchinsert}{\textsc{BatchInsert}}
\newcommand{\deleteTree}{\textsc{DeleteTree}}
\newcommand{\tagInbaNode}{\textsc{TagInbalanceNode}}
\newcommand{\castToBucket}{\textsc{CastToBucketNode}}
\newcommand{\batchdelete}{\textsc{BatchDelete}}
\newcommand{\markTomb}{\textsc{MarkTomb}}

\newcommand{\reduce}{\textsc{Reduce}}
\newcommand{\leafwrap}{\phi}
\newcommand{\skheight}{\lambda}
\newcommand{\samplerate}{\sigma}
\newcommand{\knn}{$k$-NN}
\newcommand{\numchunk}{l}
\newcommand{\os}{\sigma\xspace}
\newcommand{\levels}{\lambda\xspace}
\newcommand{\ourkdtree}{\ourtree}
\newcommand{\lc}{\mathit{lc}}
\newcommand{\rc}{\mathit{rc}}

%    Title:
\newcommand{\codeskip}{{\vspace{.05in}}}
%  \newcommand{\myparagraph}[1]{\noindent\emp{#1} \quad}

%    Others:
\newcommand{\mathtext}[1]{{\mathit{#1}}}
%  \newcommand{\fname}[1]{\textit{#1}}
%\newcommand{\textfunc}[1]{\mf{#1}}
%\newcommand{\nodecircle}[1]{{\textcircled{\footnotesize{#1}}}}
%\newcommand{\variablename}[1]{{\texttt{#1}}}

%    Math
\newcommand{\bmath}[1]{\bm{#1}}

%%%%%%%%%%%%%%%%%%%%
% general
%%%%%%%%%%%%%%%%%%%%
\newcommand{\true}{\emph{true}\xspace}
\newcommand{\false}{\emph{false}\xspace}
\newcommand{\True}{\textsc{True}\xspace}
\newcommand{\False}{\textsc{False}\xspace}
\newcommand{\zero}{\textit{zero}\xspace}
\newcommand{\one}{\textit{one}\xspace}


%%%%%%%%%%%%%%%%%%%%
% Our terms
%%%%%%%%%%%%%%%%%%%%
%    Common
\newcommand{\pre}{\mathit{pre}\xspace}
\newcommand{\parent}{\mathit{parent}\xspace}
\newcommand{\degree}{\mathit{degree}\xspace}
\newcommand{\flag}{\mathit{flag}\xspace}
\newcommand{\frontier}{frontier\xspace}
\newcommand{\dg}{dependence graph\xspace}
\newcommand{\DG}{DG\xspace}
\newcommand{\mathpivot}{\mathit{pivot}\xspace}
\newcommand{\element}{element\xspace}
\newcommand{\object}{object\xspace}
\newcommand{\augv}{\mathit{aug}}
\newcommand{\val}{\mathit{value}}
\newcommand{\update}{\mathit{update}}
\newcommand{\ff}{\mathcal{F}}


%    Problem
\newcommand{\phaseparallel}{phase-parallel}
\newcommand{\compatible}{compatible\xspace}
\newcommand{\incompatible}{incompatible\xspace}
\newcommand{\mis}{\mathit{MFS}}
\newcommand{\mfs}{\mis}
\newcommand{\rank}{\mathit{rank}}
\newcommand{\textrank}{rank\xspace}
\newcommand{\feasible}{feasible\xspace}
\newcommand{\ready}{ready\xspace}
\newcommand{\unready}{unready\xspace}
\newcommand{\finished}{finished\xspace}
\newcommand{\unfinished}{unfinished\xspace}
\newcommand{\obj}{\mathit{obj}}
\newcommand{\setfam}{\mathcal{F}}
%\newcommand{\ind}{\mathit{ind}}
\newcommand{\ind}{\mathcal{I}}
\newcommand{\curset}{T\xspace}
\newcommand{\dpvalue}{DP value\xspace}
\newcommand{\DPvalue}{DP value\xspace}
\newcommand{\MFS}{MFS\xspace}
\newcommand{\block}{block\xspace}
\newcommand{\pred}{\mathcal{P}}
\newcommand{\rankbar}{\overline{\rank}}
\newcommand{\relaxedrank}{relaxed rank}

%    LIS
\newcommand{\mathdp}{\mathit{dp}\xspace}
\newcommand{\mathpre}{\mathit{pre}\xspace}
\newcommand{\mathrange}{\mathit{range}\xspace}
\newcommand{\mathfirst}{\mathit{first}\xspace}
\newcommand{\mathsecond}{\mathit{second}\xspace}
\newcommand{\leftmin}{\mathit{LMin}\xspace}
\newcommand{\trange}{T_\mathrange}
\newcommand{\tpivot}{T_\mathpivot}
\newcommand{\lislength}{k}
\newcommand{\prefixminfunc}{\textsc{PrefixMin}}
\newcommand{\processfrontier}{\textsc{ProcessFrontier}}
\newcommand{\prefixmin}{{prefix-min}}
\newcommand{\swgs}{SWGS}
\newcommand{\relevant}{relevant}

%    Data Structure
\newcommand{\pabst}{PA-BST\xspace}

%    Activity selection
\newcommand{\timeend}{e}
\newcommand{\timestart}{s}
\newcommand{\ay}{A_{p_x}}
\newcommand{\ax}{A_x}
\newcommand{\leading}{pivot\xspace}


%    MIS
\newcommand{\tastree}{TAS tree\xspace}
\newcommand{\neighbor}{\mathcal{N}\xspace}
\newcommand{\dmax}{d_{\mathit{max}}\xspace}



%%%%%%%%%%%%%%%%%%%%
% Function names:
%%%%%%%%%%%%%%%%%%%%
\newcommand{\splitn}{\mf{Split}\xspace}
\newcommand{\addmark}{\mf{Mark}\xspace}
\newcommand{\addmarkbold}{\mf{\textbf{Mark}}\xspace}
\newcommand{\extract}{\mf{Extract}\xspace}
\newcommand{\boldextract}{\textbf{\textsc{Extract}}\xspace}
\newcommand{\traverse}{\mf{ExtractFrom}\xspace}
\newcommand{\collect}{\mf{Reduce}\xspace}
\newcommand{\extcond}{\mf{ExtDist}\xspace}
\newcommand{\finishcond}{\mf{FinishCheck}\xspace}
\newcommand{\boldextcond}{\mf{\bf ExtDist}\xspace}
\newcommand{\boldfinishcond}{\mf{\bf FinishCheck}\xspace}
\newcommand{\seq}{\mathit{seq}\xspace}
\newcommand{\inQ}{\mathit{inQ}\xspace}
\newcommand{\intersection}{\fname{Intersection}}
\newcommand{\union}{\fname{Union}}
\newcommand{\difference}{\fname{Difference}}
\newcommand{\intersect}{\intersection}
\newcommand{\diff}{\fname{Diff.}}
\newcommand{\multifind}{\textfunc{Multi-Find}\xspace}
\newcommand{\multiinsert}{\textfunc{Multi-Insert}\xspace}
\newcommand{\multidelete}{\textfunc{Multi-Delete}\xspace}
\newcommand{\multiupdate}{\textfunc{Multi-Update}\xspace}


%%%%%%%%%%%%%%%%%%%%
% Binary Forking / other cost models:
%%%%%%%%%%%%%%%%%%%%
\newcommand{\forkins}{\texttt{fork}}
\newcommand{\joinins}{\texttt{join}}
\newcommand{\insend}{\texttt{end}}
\newcommand{\allocateins}{\texttt{allocate}}
\newcommand{\freeins}{\texttt{free}}
\newcommand{\thread}{thread}
\newcommand{\bfmodel}{binary-forking model}
\newcommand{\MPC}[0]{\ensuremath{\mathsf{MPC}}}
\newcommand{\spanc}{span\xspace}
\newcommand{\depth}{span\xspace}
\newcommand{\TAS}{$\mf{TAS}$\xspace}
\newcommand{\TS}{$\texttt{TS}$\xspace}
\newcommand{\tas}{{\texttt{test\_and\_set}}\xspace}
\newcommand{\faa}{{\texttt{fetch\_and\_add}}\xspace}
\newcommand{\cas}{{\texttt{compare\_and\_swap}}\xspace}
\newcommand{\ati}{{\texttt{atomic\_inc}}\xspace}
\newcommand{\WriteMin}{\mf{WriteMin}\xspace}
\newcommand{\writemin}{\WriteMin}

%%%%%%%%%%%%%%%%%%%%
% Math
%%%%%%%%%%%%%%%%%%%%
%    integer/real number Sets:
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
%    Some letters:
\newcommand{\mathd}{\mathcal{D}\xspace}
\newcommand{\mathq}{\mathcal{Q}\xspace}
\newcommand{\mathc}{\mathcal{C}\xspace}
%    Thm environment:
\newtheorem{conjuncture}{Conjuncture}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{definition}{Definition}[section]

%%%%%%%%%%%%%%%%%%%%
% notes and comments
%%%%%%%%%%%%%%%%%%%%
\newcommand{\otherway}[1]{{{\color{blue}{another way to say: #1}}}}
\newcommand{\ifconference}{{{\ifx\fullversion\undefined}}}
\newcommand{\iffullversion}{{{\unless\ifx\fullversion\undefined}}}

%\makeatletter
%\def\dfnt@space@setup{%
%  \dfnt@preskip=\parskip
%    \dfnt@postskip=0pt}
%\makeatother

%%\let\proof\relax
%%\let\endproof\relax
%%\usepackage{amsthm} %http://ctan.org/pkg/amsthm
%%\newtheorem{theorem}{Theorem}
%\newtheoremstyle{exampstyle}
%  {.05in} % Space above
%  {.05in} % Space below
%  {} % Body font
%  {.5em} % Indent amount
%  {\sc \bfseries} % Theorem head font
%  {.} % Punctuation after theorem head
%  {.5em} % Space after theorem head
%  {} % Theorem head spec (can be left empty, meaning `normal')
%%\theoremstyle{exampstyle} \newtheorem{example}{Example}
%%\theoremstyle{exampstyle} \newtheorem{remark}{Remark}
%\theoremstyle{exampstyle} \newtheorem{compactdef}{Definition}
%\theoremstyle{exampstyle} \newtheorem{compactlem}{Lemma}

%\makeatletter
%\renewenvironment{proof}[1][\proofname]{\par
%  \vspace{-\topsep}% remove the space after the theorem
%  \pushQED{\qed}%
%  \normalfont
%  \topsep0pt \partopsep0pt % no space before
%  \trivlist
%  \item[\hskip\labelsep
%        \itshape
%    #1\@addpunct{.}]\ignorespaces
%}{%
%  \popQED\endtrivlist\@endpefalse
%  \addvspace{3pt plus 3pt} % some space after
%}

\newcommand{\smallsmallskip}{\vspace{.05in}}

%cref
\crefname{section}{Section}{Section}
%\crefname{theorem}{Theorem}{Theorem}
%\crefname{lemma}{Lemma}{Lemma}
%\crefname{corollary}{Corollary}{Corollary}
\crefname{table}{Table}{Table}
\crefname{figure}{Figure}{Figure}
%\Crefname{table}{Tab.}{Tab.}


==> query.tex <==
\section{Queries on \ourtree{s}\label{sec:querys}}

We note that unlike \kdtree{s} based on logarithmic method (i.e., maintaining $O(\log n)$ trees), \ourtree always maintains a single tree, so any query that applies to the classic static \kdtree works on \ourtree without any modifications.
We can, of course, carefully study the implementation details for each query, that applies to \ourtree{s} and the classic \kdtree{s}, which will be discussed in \cref{sec:impl}.
In this section, we review the analysis for queries on \kdtree{s}.

\begin{lemma}[\cite{blelloch2018geometry}]
	An orthogonal range count costs $O(2^{h(D-1)/D})$ work on a \kdtree of height $h$, and the orthogonal range query has $O(2^{h(D-1)/D}+k)$ work, where $k$ is the output size.
\end{lemma}

This indicates that when we pick $\balpara=1/O(\log n)$, the tree height is $\log n+O(1)$ (\cref{lem:tree-height}), and the range count will cost $O(n^{(D-1)/D})$, matching the best cost on a \kdtree.
Interestingly, however, in \cref{sec:exp-operation}, we show that this bound is not tight in most cases in practice.
Slightly increasing the tree height $h$ will only marginally affect the actual query cost.

The $k$-nearest neighbor (\knn) query is another typical application using \kdtree{s}.
Many theoretical analyses on the classic (single) \kdtree{s} also apply to \ourtree{s}.
For instance, one can show logarithmic expected query cost for \kdtree{s} on uniformly distributed inputs~\cite{friedman1977algorithm,sproull1991refinements}. %or on approximate range queries~\cite{arya1998optimal,maneewongvatana1999s,dickerson2000kd}.
These analyses only require asymptotic tree heights, so the bounds also apply to \ourtree{s} \whp.


\hide{

	More interestingly, we will show that under certain realistic assumptions, the $k$ nearest neighbor (\knn) query on \kdtree has an efficient cost.
	We believe this analysis is novel, and we are inspired by the analysis of \zdtree~\cite{blelloch2022parallel}.
	Here we assume a standard query algorithm that first traverse the subtree that the search point $P$ belongs; when traversing the other subtree, we prune the search if the distance between corresponding subspace of this tree node and $P$ is farther than the distance of the current $k$-th neighbor.
	The \kdtree is built by always cutting the largest dimension by object median. %, and for each tree node we know the bounding boxes of all points in this subtree.

	\begin{theorem}\label{thm:knn-query}
		Assuming $d$ and the expansion rate $\bar{c}$ as constants, finding the $k$-nearest neighbors of a point $P$ on a \kdtree{} has $O(k\log k)$ work.
	\end{theorem}
	\begin{proof}
		We will first show that the entire searching process will touch at most $O(k)$ leaves.
		Let $Q$ as the closest ancestor of the leaf containing $P$ that contains at least $k$ points.
		The search algorithm will first traverse the tree and find $k$ initial points that are all in $Q$'s subtree.
		Here $|Q|<2k$ since otherwise we will not pick $Q$.
		Let $r$ be the length of the largest dimension of $Q$'s corresponding subspace, and $r'$ be the distance from $P$ to the $k$-th nearest neighbor in $Q$.
		Based on our query algorithm, we will prune the searches if a tree node does not overlap with $B(P,r')$, which is the ball centered $P$ with radius $r'$.
		It is easy to see that $r'\le \sqrt{d}r$.

		We now argue that $B(P,r')$ contains $O(k)$ points.
		Let $Q'$ be $Q$'s ancestor that each dimension of $Q'$'s subspace is at least $r$.
		Since we always cut the \kdtree on the largest dimension, the path length between $Q'$ and $Q$ can only be at most $d-1$.
		Hence, $Q'$ subtree can contain at most $2k\cdot 2^{d-1}=O(k)$ points.
		Since $P$ is in $Q'$, the constant expansion rate $\bar{c}$ guarantees that $B(P,r)$ contains at most $\bar{c}|Q'|=O(k)$ points.
		Finally, since $r'\le \sqrt{d}r$, the constant expansion rate $\bar{c}$ again guarantees that $B(P,r')\le B(P,\sqrt{d}r)\le B(P,r)\cdot \bar{c}^{\lceil\log \sqrt{d}\rceil}=O(B(P,r))=O(k)$.
		Since the query algorithm will not touch leaves outside $B(P,r')$, the search process will visit $O(k)$ leaves.
		We can similarly show that $|B(P,\sqrt{d}r')|=O(k)$, which will be later used.

		Finally we argue that the entire search will visit $O(k)$ interior nodes.
		As shown above, the \knn{} search will eventually reach $O(k)$ leaves, and they have $O(k\log n)$ ancestors that need to be traversed and $O(k\log n)$ of their siblings that will be pruned.
		However, it is possible that some tree nodes have their subspaces overlapped with $B(P,r')$ (so they cannot be pruned) but indeed they contain no points in $B(P,r')$.
		Such visited tree nodes cannot be charged to the previous $O(k\log n)$ ones.
		For instance, \cref{fig:int-node} illustrates a 2D example with certain tree nodes in this case.
		The argument is that, we can only have $2^d+O(k)$ of such ``empty nodes'', where an empty node is a tree node that overlaps with $B(P,r')$ but with no points in it.
		The $2^d$ part is because the original traversal can touch this number of ``quadrants'' (4 in the 2d case in \cref{fig:int-node}).
		Then, every time we traverse the child of an empty node, since we always cut in the longest dimension, one side of the children (e.g., the shaded regions) must be completely in $B(P,\sqrt{d}r')$.

		Assuming $d$ is a constant, the total number of tree nodes we visit is $O(k\log n)$.
		Adding all pieces together gives the stated bound.
	\end{proof}

	\begin{SCfigure}%[t]
		\includegraphics[width=0.48\columnwidth]{figures/interior-nodes.pdf}
		%\vspace*{.1em}
		\caption{An illustration for a 2D \knn{} query that ``touches'' the subspaces of tree nodes but they contains no points in $B(P, r')$.  \label{fig:int-node}}
	\end{SCfigure}

	People have been using \kdtree on nearest neighbor searches on low dimensional spaces widely, and \cref{thm:knn-query} explains the efficiency on most real-world data that have small expansion rates.
	However, it does not contradict with the commonsense of ``curse of dimensionality''.
	For instance, a uniform distributed data roughly have $\bar{c}=2^d$, which is multiplicative in the $O(k\log k)$ bound.
	Hence, when $d$ is getting larger, the expansion rate grows exponentially, and still treating $\bar{c}$ as a constant on larger dimensions will overlook the main term.
	This is consistent with our experimental study (e.g., in \cref{table:summary}), which will be introduced in \cref{sec:exp-ext}.

}























==> range-count-table.tex <==
\begin{table}[t]
\vspace{.2em}
	\centering
	% \Huge
	% \resizebox{.4\textwidth}{!}{

	\small
	\setlength\tabcolsep{2.5pt}

	% Table generated by Excel2LaTeX from sheet 'range count'
	\begin{tabular}{c|ccc|ccc}
		\toprule
		              & \multicolumn{3}{c|}{\uniform} & \multicolumn{3}{c}{\varden}                                                                      \\
		\textbf{Dims} & \textbf{Small}                & \textbf{Medium}             & \textbf{Large} & \textbf{Small} & \textbf{Medium} & \textbf{Large} \\
		\midrule
		2             & 0.001                         & 0.008                       & 0.014          & 0.001          & 0.008           & 0.013          \\
		3             & 0.004                         & 0.032                       & 0.093          & 0.001          & 0.026           & 0.069          \\
		5             & 0.009                         & 0.212                       & 0.698          & 0.028          & 0.180           & 0.627          \\
		9             & 0.272                         & 2.18                        & 5.12           & 0.010          & 0.792           & 2.95           \\
		\bottomrule
	\end{tabular}%





	% }
	\caption{\textbf{Orthogonal range count query on our \ourlib for three types of rectangle in parallel.} The benchmark contains 100M points with dimension 3. Each type includes 10K random chosen rectangles. }
	\label{table:range-count}%
\end{table}%


==> related-work-table_mac.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{tabular}{c>{\raggedright\arraybackslash}p{4cm}>{\raggedright\arraybackslash}p{7cm}}

% \newcolumntype{J}[1]{>{\bf\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

% \begin{tabular}{cL{6cm}L{10cm}}
% \usepackage{array}

% Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{tabular}{L{1cm}|L{6cm}|L{10cm}}
% \clearpage
{
\newcolumntype{L}[1]{>{\raggedright\arraybackslash\hspace{0pt}}m{#1}}
\begin{table*}[!t]
  \small
  \centering
  %% Table generated by Excel2LaTeX from sheet 'Sheet1'
  \begin{tabular}{L{0.4cm}|L{6cm}|L{10cm}}
    % \begin{tabular}{c|p{33.75em}|p{50.585em}}
    \toprule
    & \multicolumn{1}{c|}{\textbf{General Features}}                                                                                                                                                                          & \multicolumn{1}{c}{\textbf{Existing Solutions and Their Features}}                                                                                                                                                                                                                                                                                   \\
    \midrule
    \begin{sideways}\textbf{\kdtree{}}
    \end{sideways}                         &
    \begin{itemize}[noitemsep]
      \item[$+$] Linear space
      \item[$+$] Flexible to most queries, such as \knn{} and range queries
      \item[$+$] Non-overlapping bounding boxes (thus effective pruning in queries)
      \item[$+$] Generally fast query on various distributions
      \item[$+$] Comparison-based, resistant to skewed data
      \item[$+$] Easy to generalize to more than there dimensions
      \item[$-$] Slow/complicated update
    \end{itemize}
    & \textbf{\pkdtree{}~\cite{men2025parallel}}
    \begin{itemize}[noitemsep]
      \item[$+$] I/O optimizations for construction and update
      \item[$+$] Construction with $O(n\log n)$ work and polylogarithmic span
      \item[$+$] Fastest or close to fastest query performance in most tests, except for \ods{} queries on skewed distributions
      \item[$-$] $O(m\log^2 n)$ work for batch update of batch size $m$, unfriendly to workloads with frequent updates
    \end{itemize}
    \textbf{\bhltree{} and \logtree{}~\cite{yesantharao2021parallel}}
    \begin{itemize}[noitemsep]
      \item[$+$] Can use vEB-layout for I/O optimization on queries
      \item[$+$] Construction with $O(n\log n)$ work and polylogarithmic span
      \item[$-$] $O(m\log^2n)$ (\logtree{}) or $O((n+m) \log (n+m))$ (\bhltree{}, fully rebuild) work for batch update
      \item[$-$] \logtree{} uses logarithmic method, leading to less efficient queries
    \end{itemize}\\%vpsace
    \midrule
    \multirow{2}[4]{*}{
      \begin{sideways}\textbf{\orthtree{}}
    \end{sideways}} &
    \begin{itemize}[noitemsep]
      \item[$+$] Linear space
      \item[$+$] Flexible to most queries, such as \knn{} and range queries
      \item[$+$] Non-overlapping bounding boxes (thus effective pruning in queries)
      \item[$+$] Fast queries, especially on non-skewed data
      \item[$+$] History-independent (modulo leaf wraps)
      \item[$+$] Simple/fast construction and update, especially on non-skewed data
      \item[$-$] Not resistant to skewed data
      \item[$-$] Usually not generalizable to more than three dimensions
    \end{itemize}
    & \textbf{\ourorth{} (this paper)}
    \begin{itemize}[noitemsep]
      \item[$+$] I/O optimizations for update/construction
      \item[$\star$] Fastest query performance on non-skewed data
      \item[$\star$] Generally faster updates than \pkdtree{s}, even on reasonably skewed data, but slower than \cpamtree{s}
      \item[$+$] Construction with $O(n\log n)$ work and polylogarithmic span
      \item[$\star$] $O(m\log \Delta)$ work for batch update
      \item[$-$] Most affected by skewed data in construction, update and query performance; less efficient on \ids{} queries on skewed data
    \end{itemize}
    \textbf{\zdtree{}~\cite{blelloch2022parallel}}
    \begin{itemize}[noitemsep]
      \item[$+$] Relatively resistant to skewed data due to the use of comparison sort
      \item[$+$] Construction with $O(n\log n)$ work and polylogarithmic span
      \item[$+$] $O(m\log \Delta)$ work for batch update, where $\Delta$ is the aspect ratio
      \item[$-$] Generally slower update/construction than \porth{} tree
      \item[$-$] Only work on integer coordinates and Morton curve
    \end{itemize}\\
    \midrule
    \multirow{2}[4]{*}{
      \begin{sideways}\textbf{R-tree/BVH}
    \end{sideways}}    &
    \begin{itemize}[noitemsep]
      \item[$+$] Linear Space
      \item[$+$] Very flexible rules based on object partition
      \item[$+$] Flexible to most queries, such as \knn{} and range queries
      \item[$+$] Simple/fast construction and update
      \item[$+$] Flexible to most queries, such as \knn{} and range queries
      \item[$+$] Easy to generalize to more than three dimensions
      \item[$-$] Overlapping bounding boxes (thus ineffective pruning in queries)
      \item[$-$] Usually slower queries than spatial-partition trees
    \end{itemize}
    & \textbf{\spactree{} (this paper)}
    \begin{itemize}[noitemsep]
      \item[$\star$] Compatible with Hilbert, Morton or other space filling curves
      \item[$\star$] Embedding multi-dimensional data to 1D, allowing for simple algorithm design and high parallelism (best self-speedup among tested indexes)
      \item[$+$] Construction with $O(n\log n)$ work and polylogarithmic span
      \item[$\star$] $O(m\log n)$ work and polylogarithmic span for batch update
      \item[$+$] Comparison-based, resistant to skewed data
      \item[$\star$] Fastest construction time and update time among all baselines; significant advantage on update performance
      \item[$-$] Only work on integer coordinates
      \item[$-$] Slow query performance compared to other teste indexes, due to overlapping bounding boxes
    \end{itemize}
    \textbf{Boost R-tree~\cite{schaling2011boost}}
    \begin{itemize}[noitemsep]
      \item[$+$] Various heurestics supported
      \item[$-$] No parallel construction or batch updates
      \item[$-$] Slow query performance compared to other teste indexes, due to overlapping bounding boxes
    \end{itemize}
    \\
    \midrule
    \begin{sideways}\textbf{Range-tree}
    \end{sideways}                        &
    \begin{itemize}[noitemsep]
      \item[$+$] Worst-case work bound for range queries
      \item[$-$] $O(n\log n)$ space
      \item[$-$] Only support range queries
      \item[$-$] Inefficient to generalize to more than three dimensions
    \end{itemize}
    & \textbf{CPAM/PAM range tree~\cite{sun2018pam,dhulipala2022pac}}
    \begin{itemize}[noitemsep]
      \item[$+$] Parallel construction with $O(n\log n)$ work and polylogarithmic span
      \item[$-$] No direct support for parallel batch updates
    \end{itemize}    \\
    \bottomrule
  \end{tabular}%

  \label{table:related-work}%
  \caption{A summary of the main features of different spatial trees, and existing solutions for parallel construction, update and query. ``$\star$'' marks our key technical contributions.
  In the bounds, $m$ is the batch size; $n$ is the index size, and $\Delta$ is the aspect ratio.}
\end{table*}

% \clearpage
}


==> related_works.tex <==
\section{Related Work}\label{sec:related}

We summarize the main features of different spatial trees, and existing solutions for parallel construction, update and query in \cref{table:related-work}\ziyang{change the reference name}.

..

Qi et al.~\cite{Qi2018theoretically} uses logarithmic method to enable parallel batch updates on R-trees, which maintains $O(\log n)$ trees with sizes 1, 2, ... $n/2$,
such that a batch update can be broken down into at most $O(\log n)$ tree reconstructions.
However, logarithmic method significantly increases query time, as queries need to examine $O(\log n)$ trees. A study on \kdtree{s} shows that logarithmic method may slow down queries by 5x or more.

\myparagraph{GPU-based Parallel Rtrees.}
GPU-based Parallel R-tree Construction and Querying~\cite{prasad2015gpu} (static parallel build based on Z-Curve, and parallel query on GPU).
Parallel implementation of R-trees on the GPU~\cite{luo2012parallel} (sort based on x dimension, one gpu block perform one query).

\myparagraph{Lock-based Concurrent Rtrees.}
A Study of Concurrent Operations on R-Trees~\cite{chenhhc97concurrent} (Disk based Rtree achieve concurrent control by locks).
The R-Link Tree: {A} Recoverable Index Structure for Spatial Data~\cite{ngk94rlink} (Concurrent rtree with lock in insertion and deletion).

\myparagraph{Distributed Rtrees.}
Declustering Spatial Databases on a Multi-Computer Architecture~\cite{koudas96declustering},
R-tree-based data migration and self-tuning strategies in shared-nothing spatial databases~\cite{mondal2001r},
Master-Client R-Trees: {A} New Parallel R-Tree Architecture~\cite{schnitzerL99master}(distributed R-tree processing in client-server architecture).
Declustering Spatial Databases on a Multi-Computer Architecture~\cite{koudas96declustering},
A Design of Parallel R-tree on Cluster of Workstations~\cite{shuhua2000design} (distributed R-tree with every machine a separate R-tree, the insertion and deletion therefore has no conflict).

\myparagraph{Parallel Queries.}
Parallel R-trees~\cite{kamel1992parallel} (store R-tree in multi-disk system, reduce parallel query overhead).
Parallel spatial query processing on gpus using r-trees~\cite{you2013parallel} (SFC-like (sorting on 1D), with trivial parallel query (one thread one query)).

\myparagraph{Parallel Bulkloading.}
Parallel bulk-loading of spatial data~\cite{papadopoulosM03} (serial sample and partition, then parallel recurse for static build).
Sort-based parallel loading of R-trees~\cite{achakeev2012sort} (SFC based, MPC, bulk-loading ).






..

